Electron dynamics in planar radio frequency magnetron plasmas: I. The mechanism of Hall heating and the {\mu}-mode

The electron dynamics and the mechanisms of power absorption in radio-frequency (RF) driven, magnetically enhanced capacitively coupled plasmas (MECCPs) at low pressure are investigated. The device in focus is a geometrically asymmetric cylindrical magnetron with a radially nonuniform magnetic field in axial direction and an electric field in radial direction. The dynamics is studied analytically using the cold plasma model and a single-particle formalism, and numerically with the inhouse energy and charge conserving particle-in-cell/Monte Carlo collisions code ECCOPIC1S-M. It is found that the dynamics differs significantly from that of an unmagnetized reference discharge. In the magnetized region in front of the powered electrode, an enhanced electric field arises during sheath expansion and a reversed electric field during sheath collapse. Both fields are needed to ensure discharge sustaining electron transport against the confining effect of the magnetic field. The corresponding azimuthal ExB-drift can accelerate electrons into the inelastic energy range which gives rise to a new mechanism of RF power dissipation. It is related to the Hall current and is different in nature from Ohmic heating, as which it has been classified in previous literature. The new heating is expected to be dominant in many magnetized capacitively coupled discharges. It is proposed to term it the "{\mu}-mode" to separate it from other heating modes.

==> customed_settings.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
    citecolor=blue}

% Figure
\usepackage{graphicx}
\usepackage[justification=centering]{caption}
\usepackage[justification=centering]{subcaption}
%\usepackage{graphbox}

% Units
\usepackage{siunitx}
\DeclareSIUnit\gauss{G}
%\usepackage{amsmath} % for equation spit. Seems to work despite claimed incompatibility

% Table
\usepackage{booktabs}
\newcolumntype{C}{>{$}c<{$}}
\newcolumntype{L}{>{$}l<{$}}
\newcolumntype{R}{>{$}r<{$}}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}% more space line  table
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}} % return to th line in one cell of a table.
\newcommand{\specialcellCenter}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}} % return to th line in one cell of a table.
\newcommand{\specialcellLeft}[2][l]{%
  \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}} % return to th line in one cell of a table.  
  

% ref eq et fig


%\usepackage{mathtools}
\usepackage[noabbrev]{cleveref}
